By Hook or by Crook: Exposing the Diverse Abuse Tactics of Technical Support Scammers

Technical Support Scams (TSS), which combine online abuse with social engineering over the phone channel, have persisted despite several law enforcement actions. The tactics used by these scammers have evolved over time and they have targeted an ever increasing number of technology brands. Although recent research has provided insights into TSS, these scams have now evolved to exploit ubiquitously used online services such as search and sponsored advertisements served in response to search queries. We use a data-driven approach to understand search-and-ad abuse by TSS to gain visibility into the online infrastructure that facilitates it. By carefully formulating tech support queries with multiple search engines, we collect data about both the support infrastructure and the websites to which TSS victims are directed when they search online for tech support resources. We augment this with a DNS-based amplification technique to further enhance visibility into this abuse infrastructure. By analyzing the collected data, we demonstrate that tech support scammers are (1) successful in getting major as well as custom search engines to return links to websites controlled by them, and (2) they are able to get ad networks to serve malicious advertisements that lead to scam pages. Our study period of 8 months uncovered over 9,000 TSS domains, of both passive and aggressive types, with minimal overlap between sets that are reached via organic search results and sponsored ads. Also, we found over 2,400 support domains which aid the TSS domains in manipulating organic search results. Moreover, we found little overlap with domains that are reached via abuse of domain parking and URL-shortening services which was investigated previously. Thus, investigation of search-and-ad abuse provides new insights into TSS tactics and helps detect previously unknown abuse infrastructure that facilitates these scams.

==> background.tex <==
%\section{Background and Motivation}
%\label{section:background}

Refer Figure~\ref{fig:news_timeline}.
%\begin{itemize}%

%	\item Evolution of Technical Support Scams%

%	\begin{itemize}
%		\item Inbound Phone Communication (IPC) Scams.
%		\begin{figure} []
%			\centering
%			\includegraphics[width=0.85\columnwidth]{figs/ipc_trend.eps}
%			\caption{ IPC Scams in Decline }
%			\label{ fig:ipc_trend }
%		\end{figure}
%		\item Outbound Phone Communication (OPC) Scams on the rise according to report.
%		
%		\begin{itemize}%

%			\item Illustration with paths of attacks (check Terry's paper)
%			\item Screenshot of Ads description / Sr with fields%

%		\end{itemize}%

%	\end{itemize}%

%\end{itemize}

%- Add figure to illustrate the way the scam happens
%Motivation \\
%- no systematic study of this emerging threat.
%- lack of reliable, up-to-date and publicly shared blacklists of technical support scam resources inspite of the widespread existence and acknowlegement of the scam. \\
%- adaptation of defences to evolving schemes.\\
%- crowd-sourced vs network level (coverage) revelation of resources, signal amplification:

%It is also important to have automated systems in place that complement manual and crowd-sourced methods of defending against such abuse. In this work, we
%show that we are able to amplify the signal from single instances of active technical support scams to find more instances of similar abuse using network level DNS data, thereby significantly expanding the intelligence and coverage we have around technical support scams.

\begin{figure*}[]
\centering
\resizebox{.9\linewidth}{!}{
\begin{tikzpicture}[snake=zigzag, line before snake = 5mm, line after snake = 5mm]
    % draw horizontal line  
    \draw[snake] (-1.5,0) -- (0,0); 
    \draw (0,0) -- (4.5,0);
    \draw[snake] (4.5,0) -- (6,0);
    \draw (6,0) -- (15.5,0);
    \draw[snake] (15.5,0) -- (17,0);

    % draw vertical lines
    \foreach \x in {0,3.5,7,9.5,13,15.5}
      \draw (\x cm,5pt) -- (\x cm,-10pt);

    % draw nodes
    \draw (0,0) node[below=10pt, text width=2cm] {\centering FTC cites use of SEO and ADs in TSS.~\cite{ftc_tss}} node[above=10pt] {\textbf{Jan 2014}};
    \draw (3.5,0) node[below=10pt, text width=2cm] {\centering Google and FB highlight difficulty in take downs of TSS due to the use of phone channel.~\cite{trustinads_report}} node[above=10pt] {\textbf{May 2014}};
    \draw (7,0) node[below=10pt, text width=2cm] {\centering 15 million Ads 25,000 websites blocked. TSS top list of bad actors in Search Engines~\cite{bing_bad_ads_report}} node[above=10pt] {\textbf{May 2, 2016}};
    \draw (9.5,0) node[below=10pt, text width=2cm] {\centering Bing Ads bans ads from third-party tech support services~\cite{bing_tsad_ban2}} node[above=10pt] {\textbf{May 12, 2016}};
    \draw (13,0) node[below=10pt, text width=2cm] {\centering FB Customer Service Scam on Google~\cite{fbsearch}} node[above=10pt] {\textbf{Jan 2017}};
    \draw (15.5,0) node[below=10pt, text width=2cm] {\centering Tech support scams persist with crafty techniques~\cite{technetblog}} node[above=10pt] {\textbf{Apr 2017}};
    %\draw (3,0) node[below=3pt] {$  $} node[above=3pt] {$  $};
    %\draw (4,0) node[below=3pt] {$ 5 $} node[above=3pt] {$ 50 $};
    %\draw (5,0) node[below=3pt] {$ 6 $} node[above=3pt] {$ 60 $};
    %\draw (6,0) node[below=3pt] {$  $} node[above=3pt] {$  $};
    %\draw (7,0) node[below=3pt] {$ n $} node[above=3pt] {$ 10n $};
\end{tikzpicture}}
\caption{Timeline of some news events related to search-based technical support scams (TSS). \label{fig:news_timeline}}
\end{figure*}
